Hybrid-CSR: Coupling Explicit and Implicit Shape Representation for Cortical Surface Reconstruction

We present Hybrid-CSR, a geometric deep-learning model that combines explicit and implicit shape representations for cortical surface reconstruction. Specifically, Hybrid-CSR begins with explicit deformations of template meshes to obtain coarsely reconstructed cortical surfaces, based on which the oriented point clouds are estimated for the subsequent differentiable poisson surface reconstruction. By doing so, our method unifies explicit (oriented point clouds) and implicit (indicator function) cortical surface reconstruction. Compared to explicit representation-based methods, our hybrid approach is more friendly to capture detailed structures, and when compared with implicit representation-based methods, our method can be topology aware because of end-to-end training with a mesh-based deformation module. In order to address topology defects, we propose a new topology correction pipeline that relies on optimization-based diffeomorphic surface registration. Experimental results on three brain datasets show that our approach surpasses existing implicit and explicit cortical surface reconstruction methods in numeric metrics in terms of accuracy, regularity, and consistency.

==> table/ablations.tex <==
\begin{table*}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccccccccc} 
\toprule
               & \multicolumn{3}{c}{Left Pial Surface} & \multicolumn{3}{c}{Left WM Surface} & \multicolumn{3}{c}{Right Pial Surface} & \multicolumn{3}{c}{Right WM Surface}  \\ 
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
          & ASSD  & NC    & SI     & ASSD & NC    & SI & ASSD & NC    & SI & ASSD & NC    & SI             \\ 
\midrule
DeepCSR \cite{cruz2021deepcsr} & 8.08   & 3.46  & 5.01  & 7.55  & 7.44  & 2.46  & 3.76  & 7.38  & 0.703   & 0.823 & 0.824 & 0.808            \\
Vox2Cortex \cite{bongratz2022vox2cortex} & 8.08   & 3.46  & 5.01  & 7.55  & 7.44  & 2.46  & 3.76  & 7.38  & 0.703   & 0.823 & 0.824 & 0.808            \\
CortexODE \cite{ma2022cortexode} & 8.08   & 3.46  & 5.01  & 7.55  & 7.44  & 2.46  & 3.76  & 7.38  & 0.703   & 0.823 & 0.824 & 0.808            \\

\midrule
\textbf{Hybrid-CSR}           & \textbf{0.512} & \textbf{0.476} & \textbf{0.643} & 0.993 & \textbf{0.515} & \textbf{0.479} & \textbf{0.631} & 0.925 & \textbf{0.917}   & \textbf{0.873} & \textbf{0.937} & \textbf{0.923}              \\
\bottomrule
\end{tabular}
}
\caption{
% 
\textbf{Cortical Surface Reconstruction Benchmark} -- blabla
% 
} % \caption
\label{tab:ablations}
\end{table*}

==> table/benchmark_combine.tex <==
\begin{table*}[!ht]
\centering
\caption{
% 
\textbf{Cortical Surface Reconstruction Accuracy Comparison} in terms of average symmetric surface distance (ASSD) and normal consistency (NC) on ADNI and OASIS dataset. Best values are highlighted. ASSD results are in mm. All results are listed in the format "mean value $\pm$ standard deviation". \textbf{Hybrid-CSR} represents the cortical reconstruction results $\hat{M}$ without any post processing. \textbf{\qq{+TC}} and \textbf{\qq{+TC+Refine}} indicate the reconstruction cortical surfaces $\hat{M}_{tc}$ and $\hat{M}_{f}$ separately.
% 
} % \caption

(a) ANDI dataset

\vspace{0.3em}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc} 
\toprule
               & \multicolumn{2}{c}{Left Pial} 
               & \multicolumn{2}{c}{Left WM} 
               & \multicolumn{2}{c}{Right Pial} 
               & \multicolumn{2}{c}{Right WM}  \\ 
               
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
          Method & ASSD $\downarrow$  & NC $\uparrow$      & ASSD $\downarrow$ & NC $\uparrow$   & ASSD $\downarrow$ & NC $\uparrow$   & ASSD $\downarrow$ & NC $\uparrow$                 \\ 
\midrule
DeepCSR~\cite{cruz2021deepcsr}  & .368 $\pm .082$   & .908 $\pm .015$  & .390 $\pm .162$  & .934 $\pm .016$  & .394 $\pm .083$  & .914 $\pm .012$  & .388 $\pm .172$  & .936 $\pm .014$             \\
Vox2Cortex~\cite{bongratz2022vox2cortex} & .339 $\pm .055$   & .918 $\pm .010$  & .346 $\pm .073$  & .926 $\pm .011$  & .350 $\pm .037$  & .915 $\pm .009$  & .335 $\pm .061$  & .927 $\pm .010$             \\
CorticalFlow++~\cite{lebrat2021corticalflow} & .296 $\pm .079$   & .925 $\pm .011$  & .271 $\pm .071$  & .936 $\pm .009$  & .270 $\pm .044$  & .924 $\pm .010$  & .268 $\pm .073$  & .933 $\pm .009$             \\
CortexODE~\cite{ma2022cortexode} & .258 $\pm .073$   & .929 $\pm .010$  & \textbf{.234} $\pm .064$  & .938 $\pm .010$  & .214 $\pm .035$  & .927 $\pm .009$  & \textbf{.231} $\pm .052$  & .939 $\pm .009$            \\
\cmidrule(lr){1-9}
Hybrid-CSR (ours)           & .254 $\pm .054$   & .886 $\pm .012$  & .264 $\pm .055$  & .899 $\pm .010$  & .250 $\pm .041$  & .886 $\pm .012$  & .257 $\pm .045$  & .901 $\pm .010$              \\
+ TC          & .267 $\pm .056$   & .926 $\pm .010$  & .268 $\pm .056$  & \textbf{.939} $\pm .010$  & .262 $\pm .042$  & .926 $\pm .010$  & .260 $\pm .046$  & .940 $\pm .010$            \\
+ TC + Refine          & \textbf{.203} $\pm .049$   & \textbf{.935} $\pm .009$  & .244 $\pm .056$  & \textbf{.939} $\pm .010$  & \textbf{.200} $\pm .034$  & \textbf{.935} $\pm .008$  & .240 $\pm .043$  & \textbf{.941} $\pm .010$     \\ 
\bottomrule
% \vspace{-0.8em}
\end{tabular}
}

\vspace{1em}

(b) OASIS dataset

\vspace{0.3em}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccc} 
\toprule
               & \multicolumn{2}{c}{Left Pial} 
               & \multicolumn{2}{c}{Left WM} 
               & \multicolumn{2}{c}{Right Pial} 
               & \multicolumn{2}{c}{Right WM}  \\ 
               
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
          Method & ASSD $\downarrow$  & NC $\uparrow$      & ASSD $\downarrow$ & NC $\uparrow$   & ASSD $\downarrow$ & NC $\uparrow$   & ASSD $\downarrow$ & NC $\uparrow$               \\ 
\midrule
DeepCSR  & .424 $\pm .075$   & .898 $\pm .016$  & .312 $\pm .124$  & .941 $\pm .010$  & .444 $\pm .087$  & .895 $\pm .018$  & .344 $\pm .158$  & .941 $\pm .011$            \\
Vox2Cortex & .401 $\pm .040$   & .900 $\pm .012$  & .302 $\pm .037$  & .928 $\pm .008$  & .405 $\pm .044$  & .898 $\pm .012$  & .303 $\pm .042$  & .929 $\pm .009$            \\
CorticalFlow++ ~~~~~~~~ & .326 $\pm .058$   & .913 $\pm .011$  & .225 $\pm .038$  & .937 $\pm .007$  & .318 $\pm .057$  & .913 $\pm .011$  & .227 $\pm .046$  & .935 $\pm .008$            \\
CortexODE & .279 $\pm .052$   & .919 $\pm .009$  & \textbf{.183} $\pm .036$  & \textbf{.943} $\pm .007$  & .280 $\pm .052$  & .918 $\pm .010$  & \textbf{.182} $\pm .052$  & \textbf{.943} $\pm .008$            \\
\cmidrule(lr){1-9}
Hybrid-CSR (ours)         & .298 $\pm .045$   & .879 $\pm .013$  & .220 $\pm .039$  & .905 $\pm .008$  & .301 $\pm .049$  & .880 $\pm .013$  & .218 $\pm .047$  & .907 $\pm .009$              \\
+ TC          & .311 $\pm .045$   & .915 $\pm .011$  & .220 $\pm .039$  & .941 $\pm .008$  & .313 $\pm .049$  & .915 $\pm .012$  & .219 $\pm .046$  & .942 $\pm .009$            \\
+ TC + Refine           & \textbf{.274} $\pm .043$   & \textbf{.921} $\pm .010$  & .198 $\pm .035$  & \textbf{.943} $\pm .008$  & \textbf{.275} $\pm .052$  & \textbf{.920} $\pm .010$  & .199 $\pm .033$  & \textbf{.943} $\pm .008$     \\ 
\bottomrule
\vspace{-0.8em}
\end{tabular}
}



% \caption{
% % 
% \textbf{Cortical Surface Reconstruction Accuracy Comparison} in terms of average symmetric surface distance (ASSD) and normal consistency (NC) on ADNI and OASIS dataset. Best values are highlighted. ASSD results are in mm. All results are listed in the format "mean value $\pm$ standard deviation". \textbf{Hybrid-CSR} represents the cortical reconstruction results $\hat{M}$ without any post processing. \textbf{\qq{+TC}} and \textbf{\qq{+TC+Refine}} indicate the reconstruction cortical surfaces $\hat{M}_{tc}$ and $\hat{M}_{f}$ separately.
% % 
% } % \caption
\label{tab:benchmark}
\end{table*}

==> table/benchmark_oasis.tex <==
\begin{table*}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccccc} 
\toprule
               & \multicolumn{3}{c}{Left Pial} 
               & \multicolumn{3}{c}{Left WM} 
               & \multicolumn{3}{c}{Right Pial} 
               & \multicolumn{3}{c}{Right WM}  \\ 
               
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
          Method & ASSD  & NC    & SI     & ASSD & NC    & SI & ASSD & NC    & SI & ASSD & NC    & SI             \\ 
\midrule
DeepCSR  & .088 $\pm .01$   & .088 $\pm .01$  & .088 $\pm .01$  & .088 $\pm .01$  & .088 $\pm .01$  & .088 $\pm .01$  & .088 $\pm .01$  & .088 $\pm .01$  & .088 $\pm .01$   & .088 $\pm .01$ & .088 $\pm .01$ & .088 $\pm .01$            \\
Vox2Cortex  & 8.08   & 3.46  & 5.01  & 7.55  & 7.44  & 2.46  & 3.76  & 7.38  & 0.703   & 0.823 & 0.824 & 0.808            \\
CorticalFlow++ & 8.08   & 3.46  & 5.01  & 7.55  & 7.44  & 2.46  & 3.76  & 7.38  & 0.703   & 0.823 & 0.824 & 0.808            \\
CortexODE & 8.08   & 3.46  & 5.01  & 7.55  & 7.44  & 2.46  & 3.76  & 7.38  & 0.703   & 0.823 & 0.824 & 0.808            \\
\cmidrule(lr){1-13}
Hybrid-CSR           & \textbf{0.512} & \textbf{0.476} & \textbf{0.643} & 0.993 & \textbf{0.515} & \textbf{0.479} & \textbf{0.631} & 0.925 & \textbf{0.917}   & \textbf{0.873} & \textbf{0.937} & \textbf{0.923}              \\
+ TC          & \textbf{0.512} & \textbf{0.476} & \textbf{0.643} & 0.993 & \textbf{0.515} & \textbf{0.479} & \textbf{0.631} & 0.925 & \textbf{0.917}   \textbf{0.873} & \textbf{0.937} & \textbf{0.923}              \\
+ TC + Refine           & \textbf{0.512} & \textbf{0.476} & \textbf{0.643} & 0.993 & \textbf{0.515} & \textbf{0.479} & \textbf{0.631} & 0.925 & \textbf{0.917}   & \textbf{0.873} & \textbf{0.937} & \textbf{0.923}     \\ 
\bottomrule
\end{tabular}
}
\caption{
% 
\textbf{Cortical Surface Reconstruction Benchmark on OASIS dataset} -- blabla
% 
} % \caption
\label{tab:benchmark-oasis}
\end{table*}

==> table/pre-trained_cfpp.tex <==
\begin{table*}[!ht]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccccc} 
\toprule
               & \multicolumn{3}{c}{Left Pial} 
               & \multicolumn{3}{c}{Left WM} 
               & \multicolumn{3}{c}{Right Pial} 
               & \multicolumn{3}{c}{Right WM}  \\ 
               
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
          Dataset & ASSD  & NC    & SI     & ASSD & NC    & SI & ASSD & NC    & SI & ASSD & NC    & SI             \\ 
\midrule          
ADNI  & .178   & .938  & .063  & .214  & .943  & .013  & .174  & .938  & .086   & .212 & .942 & .026            \\
OASIS & .326   & .913  & .147  & .225  & .937  & .054  & .318  & .913  & .192   & .227 & .935 & .076           \\
\bottomrule
\end{tabular}
}
\caption{
% 
\textbf{Cortical Surface Reconstruction from Pre-trained CorticalFlow++}
% 
} % \caption
\label{tab:pre-trained_cfpp}
\end{table*}

==> table/self-intersection.tex <==
\begin{table}
%\setlength{\tabcolsep}{4.6pt} % Reduce white-space between columns, SHOULD BE SET AFTER TABLE IS FINISHED
\centering
\caption{
\textbf{Cortical Surface Reconstruction Regularity Comparison} in terms of self-intersection face ratio (SI).
}
\label{tab:self-intersection}
(a) ANDI dataset

\vspace{0.3em}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
    \toprule
        Method & Left Pial & Left WM & Right Pial & Right WM  \\
    \midrule
        DeepCSR & 0   & 0  & 0  & 0 \\
        Vox2Cortex & .741 $\pm .221$   & .719 $\pm .214$  & 1.025 $\pm .237$  & .745 $\pm .199$ \\
        CorticalFlow++ & .164 $\pm .093$   & .058 $\pm .032$  & .187 $\pm .104$  & .067 $\pm .032$ \\
        CortexODE & .112 $\pm .072$   & .013 $\pm .011$  & .173 $\pm .091$  & .004 $\pm .005$ \\
    \midrule
        Hybrid-CSR (ours) & 0   & 0  & 0  & 0 \\
        + TC  & 0   & 0  & 0  & 0 \\
        + TC + Refine & .090 $\pm .075$   & .042 $\pm .025$  & .080 $\pm .071$  & .011 $\pm .010$ \\
    \bottomrule
    \vspace{-0.8em}
\end{tabular}
}

\vspace{0.5em}
(b) OASIS dataset

\vspace{0.3em}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
    \toprule
        Method & Left Pial & Left WM & Right Pial & Right WM  \\
    \midrule
        DeepCSR & 0   & 0  & 0  & 0 \\
        Vox2Cortex & 1.110 $\pm .270$   & .994 $\pm .193$  & 1.321 $\pm .252$  & 1.022 $\pm .186$ \\
        CorticalFlow++ & .147 $\pm .100$   & .054 $\pm .060$  & .192 $\pm .123$  & .076 $\pm .068$ \\
        CortexODE & .277 $\pm .096$   & .032 $\pm .025$  & .151 $\pm .060$  & .022 $\pm .020$ \\
    \midrule
        Hybrid-CSR (ours) & 0   & 0  & 0  & 0 \\
        + TC  & 0   & 0  & 0  & 0 \\
        + TC + Refine & .034 $\pm .022$   & .040 $\pm .022$  & .029 $\pm .018$  & .037 $\pm .026$ \\
    \bottomrule
    \vspace{-0.8em}
\end{tabular}
}

% \vspace{0.5em}


\end{table}
